Adaptive functional principal components analysis

Functional data analysis almost always involves smoothing discrete observations into curves, because they are never observed in continuous time and rarely without error. Although smoothing parameters affect the subsequent inference, data-driven methods for selecting these parameters are not well-developed, frustrated by the difficulty of using all the information shared by curves while being computationally efficient. On the one hand, smoothing individual curves in an isolated, albeit sophisticated way, ignores useful signals present in other curves. On the other hand, bandwidth selection by automatic procedures such as cross-validation after pooling all the curves together quickly become computationally unfeasible due to the large number of data points. In this paper we propose a new data-driven, adaptive kernel smoothing, specifically tailored for functional principal components analysis through the derivation of sharp, explicit risk bounds for the eigen-elements. The minimization of these quadratic risk bounds provide refined, yet computationally efficient bandwidth rules for each eigen-element separately. Both common and independent design cases are allowed. Rates of convergence for the estimators are derived. An extensive simulation study, designed in a versatile manner to closely mimic the characteristics of real data sets supports our methodological contribution. An illustration on a real data application is provided.

==> sections3/real_data_sunny.tex <==
% !TeX root = ../main_KPW_SM_proof.tex


\section{Real data application}\label{lets_see}
We return to the household electricity consumption data set, first seen in Section \ref{subsec:dgp_1}. In order to preserve the independence between curves and avoid issues with seasonality, we extracted the voltage curves in the month of June for analysis, corresponding to a summer month in France (analysis for January, a winter month, is provided in the Supplementary Material). This resulted in 119 curves with 1440 sampling points along each curve, corresponding to voltage consumption at each minute. After removing curves with incomplete or missing data, the final dataset contained 109 curves. We note that even with 1440 sampling points along each curve, the curves are still likely to be considered sparse, due to their low regularity, in the sense that $\mathfrak{m}^{2\underline H} < N$. In order to perform comparisons with sampling points following a random design, we first drew the number of points along each curve $M_i$ from a poisson distribution, with mean parameter $\mathfrak m \in \{25, 50\}$. $M_i$ points were then randomly sampled from each curve $i$ from a uniform distribution. Since there were problems with discrete sampling in the approach of \cite{Zhang2016} in the package \cite{Zhou2022} due to sampling points along each curve being equal after pooling which causes errors, we sampled points $T_m^{(i)}$'s from a continuous uniform distribution on $[0, 1]$ instead. The closest observed points to the simulated sampling points were then selected. For our approach, we used very much the same parameter settings as in the simulations, performing FPCA on a grid of 101 equally spaced points, with the same bandwidth and parameter grids. Comparisons were then made to the approach of \cite{Zhang2016} with both the default bandwidth and with generalised cross-validation, and the results can be seen in Figure \ref{efun_application_june} and Tables \ref{eval_june_m25} and \ref{eval_june_m50}. Plots comparing the computational times are given in 


\begin{figure}
\caption{Eigenfunction plots in the real data application comparing our method (WPK) to \cite{Zhou2022} with generalised cross-validation and the default bandwidth setting.}
\label{efun_application_june}
\includegraphics[scale=0.7]{sections3/electricity_app/june/plots/psi_m25_june.pdf}
\includegraphics[scale=0.7]{sections3/electricity_app/june/plots/psi_m50_june.pdf}
\end{figure}

\begin{table}[ht]
\centering
\caption{Eigenvalues for $\mathfrak{m} = 25$.}
\label{eval_june_m25}
\begin{tabular}{rrrrrrrrrrr}
  \hline
 & $\lambda_1$ & $\lambda_2$ & $\lambda_3$ & $\lambda_4$ & $\lambda_5$ & $\lambda_6$ & $\lambda_7$ & $\lambda_8$ & $\lambda_9$ & $\lambda_{10}$ \\ 
  \hline
WPK & 3.27 & 0.31 & 0.18 & 0.06 & 0.04 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  ZW & 3.66 & 0.33 & 0.29 & 0.10 & 0.06 & 0.03 & 0.02 & 0.01 & 0.01 & 0.00 \\ 
  ZW\_default & 3.63 & 0.31 & 0.20 & 0.03 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
   \hline
\end{tabular}
\end{table}


\begin{table}[ht]
\centering
\caption{Eigenvalues for $\mathfrak{m} = 50$}
\label{eval_june_m50}
\begin{tabular}{rrrrrrrrrrr}
  \hline
 & $\lambda_1$ & $\lambda_2$ & $\lambda_3$ & $\lambda_4$ & $\lambda_5$ & $\lambda_6$ & $\lambda_7$ & $\lambda_8$ & $\lambda_9$ & $\lambda_{10}$ \\ 
  \hline
WPK & 3.35 & 0.28 & 0.21 & 0.11 & 0.11 & 0.06 & 0.02 & 0.02 & 0.00 & 0.01 \\ 
  ZW & 3.35 & 0.35 & 0.25 & 0.21 & 0.16 & 0.12 & 0.09 & 0.06 & 0.05 & 0.03 \\ 
  ZW\_default & 3.20 & 0.21 & 0.15 & 0.08 & 0.03 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 \\ 
   \hline
\end{tabular}
\end{table}










